Multimodal Semi-Supervised Learning for Text Recognition

Until recently, the number of public real-world text images was insufficient for training scene text recognizers. Therefore, most modern training methods rely on synthetic data and operate in a fully supervised manner. Nevertheless, the amount of public real-world text images has increased significantly lately, including a great deal of unlabeled data. Leveraging these resources requires semi-supervised approaches; however, the few existing methods do not account for vision-language multimodality structure and therefore suboptimal for state-of-the-art multimodal architectures. To bridge this gap, we present semi-supervised learning for multimodal text recognizers (SemiMTR) that leverages unlabeled data at each modality training phase. Notably, our method refrains from extra training stages and maintains the current three-stage multimodal training procedure. Our algorithm starts by pretraining the vision model through a single-stage training that unifies self-supervised learning with supervised training. More specifically, we extend an existing visual representation learning algorithm and propose the first contrastive-based method for scene text recognition. After pretraining the language model on a text corpus, we fine-tune the entire network via a sequential, character-level, consistency regularization between weakly and strongly augmented views of text images. In a novel setup, consistency is enforced on each modality separately. Extensive experiments validate that our method outperforms the current training schemes and achieves state-of-the-art results on multiple scene text recognition benchmarks.

==> tables/fusion_augs_ablation.tex <==
\begin{table*}[t] 
% \captionsetup{font=tiny}
  \tabcolsep=0.13cm
    \begin{center}
    \caption{\textbf{Two-Stage vs. Unified Vision Model Pretraining.} Accuracy attained by both the pretrained VM and the fine-tuned ABINet, using Two-Stage and Unified pretraining, on the common and non-common datasets (average results)
    }
    \label{sup-tab:fusion_aug_ablation}
        \begin{adjustbox}{width=0.7\linewidth}
        \begin{tabular}{@{}cccc@{}}
            \toprule
            \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Augmentations}} & \textbf{Common} & \textbf{Non-Common} \\
            & &  \textbf{Benchmarks} & \textbf{Benchmarks} \\
            \midrule
            \textit{Supervised Baseline}~\cite{abinet_fang2021read} & ABINet~\cite{abinet_fang2021read} & 85.3 & 57.9 \\
            Ours & SeqCLR~\cite{seqclr_aberdam2021sequence} & ? & ? \\
            Ours & Our-HC & ? & ? \\
            Ours & Ours & ? & ? \\
            \bottomrule
        \end{tabular}
        \end{adjustbox}
    \end{center}
\end{table*} 
